Fine-Grained Urban Flow Inference

The ubiquitous deployment of monitoring devices in urban flow monitoring systems induces a significant cost for maintenance and operation. A technique is required to reduce the number of deployed devices, while preventing the degeneration of data accuracy and granularity. In this paper, we present an approach for inferring the real-time and fine-grained crowd flows throughout a city based on coarse-grained observations. This task exhibits two challenges: the spatial correlations between coarse- and fine-grained urban flows, and the complexities of external impacts. To tackle these issues, we develop a model entitled UrbanFM which consists of two major parts: 1) an inference network to generate fine-grained flow distributions from coarse-grained inputs that uses a feature extraction module and a novel distributional upsampling module; 2) a general fusion subnet to further boost the performance by considering the influence of different external factors. This structure provides outstanding effectiveness and efficiency for small scale upsampling. However, the single-pass upsampling used by UrbanFM is insufficient at higher upscaling rates. Therefore, we further present UrbanPy, a cascading model for progressive inference of fine-grained urban flows by decomposing the original tasks into multiple subtasks. Compared to UrbanFM, such an enhanced structure demonstrates favorable performance for larger-scale inference tasks.

==> table/minipage.tex <==
\begin{figure}
\begin{minipage}[b]{0.22\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/fig_percentage.png}
  \caption{figure}
  \vspace{-0.8em}
\end{minipage}
%\hfill
\begin{minipage}[b]{0.22\textwidth}
  \centering
  \small
  \tabcolsep=1mm
  \begin{tabular}{lcccc}\hline
    Method & 10 & 30 & 50 & 100\\ \hline
    SRResNet & 20 & 20 & 20 & 20  \\
    SRResNet-CL & 20 & 20 & 20 & 20\\
    UrbanFM & 20 & 20 & 20 & 20\\
    UrbanFM-NE  &20 & 20 & 20 &20\\\hline
    \end{tabular}
    \vspace{5mm}
    \caption{table}
  \end{minipage}
\end{figure}
%\end{minipage}

==> table/overall-taxi.tex <==
% Table generated by Excel2LaTeX from sheet 'overall-taxi'
\begin{table*}[!t]
  \centering
  %\small
  \caption{\label{tab:main_bj}Results comparisons on TaxiBJ over different time spans (P1-P4).}
  \vspace{-0.8em}
  \tabcolsep=0.22cm
    \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \shline
    \multirow{2}*{Methods} & \multicolumn{3}{c|}{P1} & \multicolumn{3}{c|}{P2} & \multicolumn{3}{c|}{P3} & \multicolumn{3}{c}{P4} \\
\cline{2-13}           & RMSE  & MAE   & MAPE  & RMSE  & MAE   & MAPE  & RMSE  & MAE   & MAPE  & RMSE  & MAE   & MAPE \\
    \hline
    MEAN  & 20.918 & 12.019 & 4.469 & 20.918 & 12.019 & 5.364 & 27.442 & 16.029 & 5.612 & 19.049 & 11.070 & 4.192 \\

    HA    & 4.741 & 2.251 & 0.336 & 5.381 & 2.551 & 0.334 & 5.594 & 2.674 & 0.328 & 4.125 & 2.023 & 0.323 \\
    \hline
    SRCNN & 4.297 & 2.491 & 0.714 & 4.612 & 2.681 & 0.689 & 4.815 & 2.829 & 0.727 & 3.838 & 2.289 & 0.665 \\

    ESPCN & 4.206 & 2.497 & 0.732 & 4.569 & 2.727 & 0.732 & 4.744 & 2.862 & 0.773 & 3.728 & 2.228 & 0.711 \\

    DeepSD & 4.156 & 2.368 & 0.614 & 4.554 & 2.612 & 0.621 & 4.692 & 2.739 & 0.682 & 3.877 & 2.297 & 0.652 \\
    \hline
    VDSR  & 4.159 & 2.213 & 0.467 & 4.586 & 2.498 & 0.486 & 4.730 & 2.548 & 0.461 & 3.654 & 1.978 & 0.411 \\

    SRResNet & 4.164 & 2.457 & 0.713 & 4.524 & 2.660 & 0.688 & 4.690 & 2.775 & 0.717 & 3.667 & 2.189 & 0.637 \\

    \hline
    UrbanFM-ne & 4.015 & 2.047 & 0.332 & 4.386 & 2.258 & 0.320 & 4.559 & 2.352 & 0.316 & 3.559 & 1.845 & 0.309 \\

    \textbf{UrbanFM} & \textbf{3.950} & \textbf{2.011} & \textbf{0.327} & \textbf{4.329} & \textbf{2.224} & \textbf{0.313} & \textbf{4.496} & \textbf{2.318} & \textbf{0.315} & \textbf{3.501} & \textbf{1.815} & \textbf{0.308} \\
    \shline

    \end{tabular}%
\end{table*}%


==> table/param.tex <==
\begin{table}[h]
	\centering
	\renewcommand{\arraystretch}{1.1}

    \begin{subfloat}[h]{
        \centering
		\begin{tabular}{c|cc|rrr}
		\shline
    	\multicolumn{1}{c|}{Methods} & \multicolumn{1}{l}{Settings} & \multicolumn{1}{l|}{\#Params} & \multicolumn{1}{l}{RMSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE} \\
		\hline
	    SRResNet & 20-64 & 1.8M  & 4.317 & 2.586 & 0.725 \\
   		UrbanFM & 20-64 & 1.9M  & 4.094 & 2.101 & 0.321 \\
    	\hline
	    SRResNet & 16-64 & 1.5M  & 4.261 & 2.520 & 0.689 \\
    	UrbanFM & 16-64 & 1.7M  & 4.107 & 2.118 & 0.322 \\
	    \hline
    	SRResNet & 16-256 & 24.2M & 4.178 & 2.418 & 0.614 \\
	    UrbanFM & 16-256 & 24.4M & 4.068 & 2.087 & 0.316 \\
    	\shline
	    \end{tabular}%
	}
    \end{subfloat}
    \hfill
    
    \begin{subfloat}[h]{
        \centering
    \begin{tabular}{c|ll|rrr}
    \shline
    Method & Settings & \#Params & RMSE & MAE & MAPE \\
    \hline
    \multirow{7}{*}{UrbanPy} & [64-4-4](base) & 4.7M  & 4.572 & 2.237 & 0.352 \\
\cline{2-6}          & [32-4-4] & 3.0M  & 4.731 & 2.326 & 0.379 \\
          & [128-4-4] & 11.6M & 4.547 & 2.222 & 0.348 \\
\cline{2-6}          & [64-8-4] & 5.6M  & 4.581 & 2.240 & 0.351 \\
          & [64-2-4] & 4.3M  & 4.619 & 2.265 & 0.359 \\
\cline{2-6}          & [64-4-1] & 3.9M  & 4.576 & 2.239 & 0.350 \\
          & [64-4-8] & 5.8M  & 4.571 & 2.233 & 0.349 \\
    \shline
    \end{tabular}
    }
     \end{subfloat}
     \caption{Max and min temps recorded in the first two weeks of July}
     \label{tab:param_study}
\end{table}


==> table/parameter_urbanpy.tex <==
% Table generated by Excel2LaTeX from sheet 'studies'
\begin{table}[htbp]
  \centering
  \renewcommand{\arraystretch}{1.1}
  \caption{Studies on different $F$-$D$-$R$ settings}
    \begin{tabular}{l|l|rrr}
    \shline
    Variants & \#Params & \multicolumn{1}{l}{RMSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE} \\
    \hline
    64-4-4~(base) & 4.7M  & 4.572 & 2.237 & 0.352 \\
    \hline
    32-4-4 & 3.0M  & 4.731 & 2.326 & 0.379 \\
    128-4-4 & 11.6M & 4.547 & 2.222 & 0.348 \\
    \hline
    64-8-4 & 5.6M  & 4.581 & 2.240 & 0.351 \\
    64-2-4 & 4.3M  & 4.619 & 2.265 & 0.359 \\
    \hline
    64-4-1 & 3.9M  & 4.576 & 2.239 & 0.350 \\
    64-4-8 & 5.8M  & 4.571 & 2.233 & 0.349 \\
    \shline
    \end{tabular}%
  \label{tab:param_urbanpy}%
\end{table}%

